Efficient Concurrent Execution of Smart Contracts in Blockchains using Object-based Transactional Memory

This paper proposes an efficient framework to execute Smart Contract Transactions (SCTs) concurrently based on object semantics, using optimistic Single-Version Object-based Software Transactional Memory Systems (SVOSTMs) and Multi-Version OSTMs (MVOSTMs). In our framework, a multi-threaded miner constructs a Block Graph (BG), capturing the object-conflicts relations between SCTs, and stores it in the block. Later, validators re-execute the same SCTs concurrently and deterministically relying on this BG. A malicious miner can modify the BG to harm the blockchain, e.g., to cause double-spending. To identify malicious miners, we propose Smart Multi-threaded Validator (SMV). Experimental analysis shows that the proposed multi-threaded miner and validator achieve significant performance gains over state-of-the-art SCT execution framework.

==> ap-objective.tex <==
%\vspace{-.5cm}
\section{Requirements of \Mthr Miner, Block Graph and Validator}
\label{apn:sti_min_bg_val}
%This section demonstrates the stipulation of concurrent miner to execute the smart contract transactions concurrently while ensuring the correctness using object semantics. %Concurrent miner constructs the block graph concurrently which maintains the dependency among smart contract transactions. Later, concurrent validators execute the smart contract transactions concurrently and deterministically with the help of block graph.
This section explores the requirements for the correct working of a \mthr miner, \mthr validator on object semantics, and the conditions of block graph. 

\vspace{1mm}
\noindent
\textbf{Requirements of the \Mthr Miner:}
\label{subsec:st_min}
A \mthr miner uses multiple threads to execute smart contract transactions (SCTs) concurrently. Thread uses STMs to handle synchronization issues. %As mentioned in \secref{intro}, Ethereum's \sctrn{s} use hash-tables extensively. Hence, hash-table based \svotm or HT-SVOSTM is very effective in this context. 

Systems executing transactions concurrently must ensure that the concurrent execution is correct. Concurrent executions can give rise to many inconsistent behaviors such as infinite loop, divide by zero error, crash failures. When the transactions are executed in a controlled environment like a virtual machine, then some of this inconsistent behavior, such as crash failures can be prevented. (Ethereum Virtual Machine or EVM execute Ethereum \sctrn{s}). But not all anomalies such as infinite loop can be prevented by the virtual machine.

The inconsistent executions can be prevented by ensuring that the executions produced by the STM system are \opq \cite{GuerKap:Opacity:PPoPP:2008} or one of its variants such as \coopty \cite{Peri+:OSTM:Netys:2018}, \lopty, or \vwc{} \cite{KuzSat:NI:TCS:2016}. In this paper, we consider \coopty and \opty as the \cc for \svotm and \mvotm respectively. 

\ignore{

%A concurrent execution of SCTs by the miner is said to be correct if there exists an equivalent serial schedule or satisfies the correctness-criteria.

An inconsistent read during concurrent execution may lead the system to severe issues such as crash failure, divide by zero, infinite loop, etc. Nowadays, SCTs execute on the virtual machine \cite{Dickerson+:ACSC:PODC:2017}. Concurrent execution of SCTs by miner may get an infinite loop and divide by zero error in the virtual machine. So, concurrent execution of SCTs by miner should ensure the correctness criteria as opacity \cite{GuerKap:Opacity:PPoPP:2008}. 

Sometimes, it is better to adapt to the non-virtual machine environment because of its better efficiency. The non-virtual machine requires the safeguard of the transactions. So, here as well to ensure the correct concurrent execution of SCTs by miner should satisfy the correctness criteria as opacity. \Mthr miner constructs the block graph (BG) concurrently to maintains the dependencies among SCTs. Later, concurrent validators execute the SCTs of this block concurrently and deterministically with the help of BG given by the miner.  

\begin{requirement}
    Any history $H_m$ generated by \mthr miner using object semantics should ensure the correctness criteria opacity.
\end{requirement}
}

%Here, concurrent miner executes the smart contract transaction using object semantics to calculate the final state and simultaneously constructs the block graph in a lock-free manner which maintains the dependency among smart contract transactions. Concurrent miner append this block graph along with the final states and proposed the block. After that, it broadcast to validators. Later, concurrent validators re-execute the smart contract transactions concurrently and deterministically with the help of block graph to validate the proposed block correctly.

\vspace{1mm}
\noindent
\textbf{Requirements of the Block Graph:} As the threads of a miner node execute the \sctrn{s} concurrently, they capture the dependencies among the \sctrn{s} in the form a block graph or BG which is stored in the block. The BG helps the validator nodes to execute the block in a multi-threaded manner. The transactions in BG which do not have any path between them are independent and can be executed concurrently by different threads. Thus by not allowing concurrent execution of dependent transactions, our system avoids \emph{false block rejection}. 

%BG captures the dependencies among the SCTs as executed by the concurrent miner and helps the validators to execute the dependent transactions in the same order to get rid of \emph{false block rejection (or FBR)}  error as explain in \secref{intro}. Concurrent validators apply topological sort on the BG and concurrently execute the SCTs which don't have any dependency in the BG.

The \blg execution by the miner and validators ensure that the history generated by \mthr validators $H_v$ is equivalent to the history generated by \mthr miner $H_m$. Only when $H_v$ is equivalent to $H_m$, can \fbr error be avoided.

Equivalence depends on the STM protocol used by the \mthr miner. If the \mthr miner uses Single-Version OSTM protocol \cite{Peri+:OSTM:Netys:2018} then $H_v$ and $H_m$ are view equivalence which can be approximated by conflict equivalence \cite[Chap. 3]{WeiVoss:TIS:2002:Morg}. So, in this case, the \blg generated by the miner will be a conflict graph \cite[Chap. 3, 6]{WeiVoss:TIS:2002:Morg}. Whereas if \mthr miner uses Multi-Version OSTM protocol \cite{Juyal+:MVOSTM:SSS:2018}, then $H_v$ and $H_m$ are multi-version view equivalent. Hence, the BG generated by the miner will be multi-version serialization graph %\cite [Chap. 5]{WeiVoss:TIS:2002:Morg}, 
\cite{Juyal+:MVOSTM:SSS:2018}.

To build the \blg, the miner threads identify the dependencies between the \sctrn{s} using the STMs that execute these \sctrn{s}. To be efficient, the graph is built in a distributed manner by threads without locks. %All these details are explained in \secref{pm}. 

% as memory transactions. To make it easy to identify the dependencies, both the single-version and multi-version \ostm{s} are based on timestamps. 
 
 
 
\vspace{1mm} 
\noindent
\textbf{Requirements of the \Mthr Validator:}
As explained above, the validator creates multiple threads to re-execute the \sctrn{s} concurrently rely on the \blg provided by the \mthr miner. Since the miner has already identified all the dependencies among the transactions, the validator threads need not worry about synchronization issues. The validator threads allow concurrent execution of \sctrn{s} that has no dependencies in the \blg. 







%Concurrent validator runs multiple threads to re-execute the SCTs concurrently and deterministically with the help of BG given by the concurrent miner. The concurrent execution by validator is said to be correct if there exists an equivalent serial schedule. Topological sort on BG provides a serial schedule. BG helps concurrent validators to execute the dependent SCTs in the same order as executed by the concurrent miner to resolve the FBR error. However, concurrent validators can execute the independent SCTs in any order. Therefore, the BG gives a partial order of the SCTs. So, concurrent validators need not to worry about any consistency issues. BG ensures the consistency while disallowing the concurrent execution of conflicting transactions.

\ignore {
\section{Requirements on Concurrent Miner and Validator}
\label{sec:req-miner_val}

This section describes the requirements of concurrent miner and validator to ensure correct concurrent execution of the \scontract transactions. 

%\todo{In one of the sections below, bring the ideas of MVE, VE \& CE.}

\subsection{Requirements of the Concurrent Miner}
The miner process invokes several threads to concurrently execute the \scontract transactions or \au{s}. With the proposed optimistic execution approach, each miner thread invokes a \au as a transaction. %It is important to ensure that the concurrent execution is \emph{correct}. 

The miner should ensure the correct concurrent execution of smart contract transactions. The incorrect concurrent execution (or consistency issues) may occur when concurrency involved. Any inconsistent read may leads system to divide by zero, infinite loops, crash failure etc. All smart contract transactions take place within a virtual machine \cite{Dickerson+:ACSC:PODC:2017}. %Virtual machine environment can get rid of the issues of inconsistent read while executing the smart contract transactions sequentially. 
When miner executes the smart contract transactions concurrently on virtual machine then infinite loop and inconsistent read may occur. So, to ensure the correct concurrent execution, miner should satisfy the correctness-criterion as opacity \cite{GuerKap:Opacity:PPoPP:2008}.

To achieve better efficiency, sometimes we need to adapt the non-virtual machine environment which necessitates with the safeguard of transactions. There as well miner needs to satisfies the correctness-criterion as opacity to ensure the correct concurrent execution of smart contract transactions. %Opacity assures that all the transactions read consistent values including aborted transactions as well. 

%In non-virtual machine environment, any inconsistent read may leads to divide by zero, infinite loops, crash failure of concurrent miner etc. So, the correct concurrent execution by miner should ensures opacity which says all the transactions read consistent values including aborted transactions as well. % The concurrent execution of the \scontract transactions of a block by the validators which although is highly desirable can further complicate the situation. 
\begin{requirement}
	Any history $H_m$ generated by concurrent miner should satisfy opacity.
\end{requirement}
\cmnt{
\begin{proof}
	Here, miner executes the smart contract concurrently with the help of optimistic STM protocols (BTO and MVTO). Internally, BTO and MVTO \cite{Kumar+:MVTO:ICDCN:2014} protocol ensures opacity. So, history $H_m$ generated Concurrent miner satisfies opacity.
\end{proof}
}

%Concurrent miner provides $BG$ to concurrent validators to ensure the correct output by validators. After that concurrent validator apply topological sort on $BG$ and generates a history $H_v$.

%Once a concurrent miner proposes a block, then validator re-executes the same set of transactions concurrently to validate it. But during the concurrent execution, suppose the validator execute two conflicting transactions in a different order from what was executed by the miner. Thus the serialization order of the miner is different from the validator. Then this can result in the validator obtaining a different final state than what was obtained by the miner. Thus the validator may incorrectly reject the block although it is valid. 

Concurrent miner maintains a BG and provide it to concurrent validators which ensures the dependency order among the conflicting transactions. As we discussed in \secref{intro}, if concurrent miner will not maintain the BG then a valid block may get rejected by the concurrent validator. %BG helps to achieve the same final state by concurrent validators as concurrent miner.


\subsection{Requirements of the Concurrent Validator}
The correct concurrent execution by validator should be equivalent to some serial execution. Serial order can be obtained by applying the topological sort on the BG provided by the concurrent miner. BG gives partial order among the transactions while restricting the dependency order same as concurrent miner. So validator executes those transactions concurrently which are not having any dependency among them with the help of BG. Validator need not have to worry about any concurrency control issues because BG ensures conflicting transactions never execute concurrently.

For validator, we can use any concurrency control mechanism to execute smart contract transactions concurrently but transactions may abort on conflict and retry. Retrying the conflicting transactions may take time which leads to slow down the performance of concurrent validator. 

%In order to improve the efficiency of concurrent validator, we consider $BG$ which allow to execute the transactions concurrently without abort.


%The correct concurrent validator execution obtains a total order among the transactions. The way, we have done the concurrent validators need not to worry about concurrency control issues.

%\subsection{Requirements of the Block Graph}
\cmnt{
Block graph ensures view equivalence between the histories of the concurrent miners and validators. During the concurrent execution of miner using STM\_BTO protocol, conflict graph (same as BG) captures the view equivalence between the histories of the concurrent miners and validators while maintaining single-version corresponding to each data-objects. We can use the STMs for the concurrent execution by validators but aborts will be there. In order to improve the efficiency of concurrent validator, we consider $BG$ which allow to execute the transactions concurrently without abort. Consider the history $H_m$ generated by STM\_BTO protocol and constructs $BG$ in which each committed transaction $T_i$ consider as vertices and edges between them as follows:
\begin{itemize}
\item r-w: If $T_j$ writes $x$ after read by $T_i$ in $H_m$, then there is an edge from $v_i$ to $v_j$. %Note that in order for this to happen, $T_i$ must have committed before $T_j$ and $c_i$ $<_{H_m}$ $w_j(x)$. 
This set of edges are referred to as r-w.
%$T_i$ reads $x$ from $T_k$, after that $T_j$ writes on $x$ data-object then r-w edge will be from $T_i$ to $T_j$.  
\item w-r: If $T_j$ reads $x$ from $T_i$ in $H_m$, then there is an edge from $v_i$ to $v_j$. Note that in order for this to happen, $T_i$ must have committed before $T_j$ and $c_i$ $<_{H_m}$ $r_j(x)$. This set of edges are referred to as w-r.
%If $T_i$ reads $x$ from the value written by $T_j$ then w-r edge will be from $T_i$ to $T_j$. 
\item w-w: If $T_j$ writes to $x$ after written by $T_i$ in $H_m$, then there is an edge from $v_i$ to $v_j$. Note that in order for this to happen, $T_i$ must have committed before $T_j$ and $c_i$ $<_{H_m}$ $w_j(x)$. This set of edges are referred to as w-w.
%If $T_i$ writes into $x$ before written by $T_j$ then w-w edge will be from $T_i$ to $T_j$. 
\item \rt(real-time) edges: If $T_j$ starts after commit of $T_i$ in $H_m$, then there is an edge from $v_i$ to $v_j$. This set of edges are referred to as $\rt(H_m)$.
\end{itemize}

Whereas when we consider the concurrent execution of miner using STM\_MVTO protocol which stores multiple version corresponding to each data-objects, conflict graph can be restrictive. So, we consider Multi-Version Serialization Graph, MVSG $(H_m,\ll)$ for a given version order of history $H_m$ as follows to ensure the multi-version view equivalence between the histories of the concurrent miners $H_m$ and validators $H_v$:
\begin{enumerate}
\item \textit{\rt}(real-time) edges: If $T_i$ commits before $T_j$ starts in $H_m$, then there is an edge from $v_i$ to $v_j$. This set of edges are referred to as $\rt(H_m)$.

\item \textit{\rf}(reads-from) edges: If $T_j$ reads $x$ from $T_i$ who has written on $x$ in $H_m$, then there is an edge from $v_i$ to $v_j$. Note that in order for this to happen, $T_i$ must have committed before $T_j$ and $c_i$ $<_{H_m}$ $r_j(x)$. This set of edges are referred to as $\rf(H_m)$.

\item \textit{\mv}(multi-version) edges: The \mv{} edges capture the multi-version relations and is based on the version order. Consider a successful read \op{} $r_k(x,v)$ and the write \op{} $w_j(x,v)$ belonging to transaction $T_j$ such that $r_k(x,v)$ reads $x$ from $w_j(x,v)$ (it must be noted $T_j$ is a committed transaction and $c_j$ $<_{H_m}$ $r_k$). Consider a committed transaction $T_i$ which writes to $x$, $w_i(x, u)$ where $u \neq v$. Thus the versions created $x_i, x_j$ are related by $\ll$. Then, if $x_i \ll x_j$ we add an edge from $v_i$ to $v_j$. Otherwise ($x_j \ll x_i$), we add an edge from $v_k$ to $v_i$. This set of edges are referred to as $\mv(H_m, \ll)$.
\end{enumerate}

\begin{lemma}
	History $H_m$ generated by MVTO protocol and $H_v$ are multi-version view equivalent.
\end{lemma}
}
}

==> ap-relatedwork.tex <==
\section{Remaining Related Work}
\label{apn:rwork}

\noindent
Nowadays, blockchain is one of the most revolutionary technology in the world. Cryptocurrencies such as Ethereum \cite{ethereum:url} and several other blockchains run the complex code known as a smart contract. Basically, there are two aspects where researchers are exploring: (1) Security aspects in which researchers are working to make the blockchain technology more secure. (2) Concurrency aspect \cite{Anjana:OptSC:PDP:2019,Bartoletti:2019arXiv190504366B,Dickerson+:ACSC:PODC:2017,ZangandZang:ECSC:WBD:2018} in which researchers are working to execute the blockchain efficiently and concurrently.

%Zang et al. \cite{ZangandZang:ECSC:WBD:2018} proposed a concurrent validator which validates the proposed block by miner using MVTO protocol. 
Zhang et al. \cite{ZangandZang:ECSC:WBD:2018} have developed a multi-threaded miner and validator solution. In their solution, the miner can use any concurrency control mechanism developed
in databases while the validator uses multi-version timestamp order (or MVTO) \cite{BernsGood:MCC:TDS:1983} based solution developed for databases. To avoid the \fbr error, the miner stores the read-write sets in the block instead of a BG. Their solution, unlike STMs, is not optimistic. Hence, they even have to re-execute committed transactions several times to ensure consistency which brings down the performance.
 Yu et al. \cite{7943307} developed a pipeline model to verify and create blocks in parallel. Yu et al. \cite{Yu:2018:PSC:3278312.3278321} proposed a parallel smart contract model which ensures better transactions processing. However, they faced synchronization issues that they resolved using transaction splitting algorithm. Dickerson et al. \cite{Dickerson+:ACSC:PODC:2017} proposed a technique in which miner executes the SCTs concurrently using pessimistic software transactional memory systems (STMs) and validator executes the SCTs concurrently using fork-join approach. Due to use of STMs Dickerson et al. need not to worry about synchronization issues, STMs takes care of it. Anjana et al. \cite{Anjana:OptSC:PDP:2019} proposed the concurrent execution of SCTs by miner using optimistic software transactional memory systems and validator executes the SCTs concurrently using the fork-join approach and decentralized approach. They considered BTO \cite [Chap. 4]{WeiVoss:TIS:2002:Morg} and MVTO protocol \cite{Kumar+:MVTO:ICDCN:2014}. %Saraph and Herlihy \cite{SaraphHerlihy:EmpSdy-Con:Arxiv:2019} proposed a speculative technique in which miner executes the SCTs which does not have any conflicts in parallel, whereas the SCTs which have conflicts in a sequential manner. 

%Pang et al. \cite{Pang:2019arXiv190507169P} proposed another technique for concurrent execution of the SCTs at miner and validator. In their work, they used a batching feature based OCC (Optimistic  Concurrency  Control) protocol at the miner. A concurrent miner also produced a schedule log and used a graph partition algorithm to break down the original schedule log into small pieces. For concurrent execution of SCTs at the validator, they used a deterministic OCC protocol and the log information shared by the miner.
A static analysis based technique for concurrent execution of the smart contract is proposed by Bartoletti et al. \cite{Bartoletti:2019arXiv190504366B}. They presented a mathematical model based statical analysis of the smart contract before executing them. In their proposed technique SCTs, they can be executed concurrently based on the semantics and swappability of the transactions. %They used OCC protocol for both miner and validator; however, if a miner generates a log then using OCC protocol at validator appears inefficient. 
All the papers, as mentioned above, have worked on the lower level operations such as read/write, and proposed solution for speculative runtime concurrent execution of the STCs by miner and validators.

%A static analysis based technique for concurrent execution of the smart contract is proposed by Bartoletti et al. \cite{Bartoletti:2019arXiv190504366B}. They presented a mathematical model based statical analysis of the smart contract before executing them. In their proposed technique SCTs, they can be executed concurrently based on the semantics and swappability of the transactions. They also claimed that their technique could be directly added in Ethereum blockchain without the requirement of any soft or hard forks to the current implementation. %However, the Ethereum Virtual Machin (EVM) is not multithreaded, so implementing any concurrent execution technique might require a soft or hard fork to the current implementation of EVM.

Herlihy et al. \cite{HerlihyKosk:Boosting:PPoPP:2008} and Peri et al. \cite{Peri+:OSTM:Netys:2018} showed that working at higher level operations provide greater concurrency, better throughput and reduces the number of aborts than the lower level. So, in this paper, we propose a novel way to execute the SCTs concurrently and efficiently by miner using higher-level object semantics SVOSTM and ensures the correctness-criteria as co-opacity. Further miner executes the SCTs concurrently through an efficient higher-level object semantics as MVOSTM and enhances the speedup while maintaining multiple versions of each shared data-items and ensure opacity. Miner constructs the BG using SVOSTM and MVOSTM protocols. Later, the proposed concurrent validators validate the block while re-executing the SCTs deterministically and concurrently using BG given by the concurrent miner.



\cmnt{


Sergey et al. \cite{SergeyandHobor:ACP:2017} elaborates a new perspective between smart contracts and concurrent objects. Zang et al. \cite{ZangandZang:ECSC:WBD:2018} uses any concurrency control mechanism for concurrent miner which delays the read until the corresponding writes to commit and ensures conflict-serializable schedule. Basically, they proposed concurrent validators using MVTO protocol with the help of write sets provided by the concurrent miner. Dickerson et al. \cite{Dickerson+:ACSC:PODC:2017} introduces a speculative way to execute smart contracts by using concurrent miner and concurrent validators. They have used pessimistic software transactional memory systems (STMs) to execute concurrent smart contracts which use rollback if any inconsistency occurs and prove that schedule generated by concurrent miner is \emph{serializable}. We proposed an efficient framework for concurrent execution of the smart contracts using optimistic software transactional memory systems. So, the updates made by a transaction will be visible to shared memory only on commit hence, rollback is not required. Our approach ensures correctness criteria as opacity \cite{GuerKap:Opacity:PPoPP:2008} which considers aborted transactions as well because it read correct values.

Weikum et al. \cite{WeiVoss:TIS:2002:Morg} proposed concurrency control techniques that maintain single-version and multiple versions corresponding to each data-object. STMs \cite{HerlMoss:1993:SigArch,ShavTou:1995:PODC} are alternative to locks for addressing synchronization and concurrency issues in multi-core systems. STMs are suitable for the concurrent executions of smart contracts without worrying about consistency issues. Single-version STMs protocol store single version corresponding to each data-object as BTO STM. It identifies the conflicts between two transactions at run-time and abort one of them and retry again for the aborted transaction. Kumar et al. \cite{Kumar+:MVTO:ICDCN:2014} observe that storing multiple versions corresponding to each data-object reduces the number of aborts and provides greater concurrency that leads to improving the throughput.
}

==> mixResults.tex <==


\ignore{

\begin{figure}[!htb]
    \centering
	\includegraphics[width=.65\textwidth]{figs/w1-w2-Speedup-mix-1.eps}\vspace{-.35cm}
	 \caption{Speedup of Concurrent Miners and SCVs for Mix Contract over Serial Miner and Validator on W1 and W2}
	\label{fig:w12-mix}
\end{figure}



\begin{figure}
	\includegraphics[width=.5\textwidth, height=4.2cm]{figs/W1MixSpeedup1.eps}\vspace{-.5cm}
	\caption{{Speedup of Concurrent Miners and Smart Concurrent Validators for Mix Contract over Serial Miner and Validator on W1}}
	%\caption{\centering Speedup of Concurrent vs Serial Miner for W1}
	\label{fig:w1-mix}
\end{figure}
%\vspace{1mm}
\begin{figure}
	\includegraphics[width=.5\textwidth, height=4.2cm]{figs/W2MixSpeedup.eps}\vspace{-.5cm}
	\caption{{Speedup of Concurrent Miners and Smart Concurrent Validators for Mix Contract over Serial Miner and Validator on W2}}
	%\caption{\centering Speedup of Concurrent vs Serial Miner for W1}
	\label{fig:w2-mix}
\end{figure}
\begin{figure}[!htb]
    \centering
	\includegraphics[width=.47\textwidth]{figs/w1-w2-mminer-mix.eps}\vspace{-.35cm}
	\caption{{\% of average concurrent validator (non SCV) accepted a malicious block for Mix Contract on W1 and W2}}
	%\caption{\centering Speedup of Concurrent vs Serial Miner for W1}
	\label{fig:w1w2mixmminer}
\end{figure}
}



==> results-new.tex <==
\section{Experimental Evaluation}
\label{sec:result}
This section presents the experimental analysis of the proposed concurrent miner and validator against state-of-the-art miners and validators. \todo{Repeated text from previous sessions, I think we can remove this.}{\color{red}Initially, we proposed the concurrent execution of SCTs by miner using \svotm protocol as \svotm miner, which maintains single-version corresponding to each shared data-item. To achieve the higher concurrency further, we introduced the concurrent execution of SCTs by miner using \mvotm protocol as \mvotm miner, which maintains multiple versions corresponding to each shared data-item.} %Since, both the STMs works on object-level, we refer these concurrent miner as object-based miner.
We compared proposed \svotm and \mvotm miner\footnote{Please find the code here: https://github.com/anonymouswin/ObjectSC} with state-of-the-art concurrent: \bto, \mvto \cite{Anjana:OptSC:PDP:2019}, Speculative Bin, Static Bin \cite{SaraphHerlihy:EmpSdy-Con:Arxiv:2019}, and Serial miner. The results show that the proposed \svotm and \mvotm miners achieve significant performance gain over \bto, \mvto, and serial miners. The STMs (\svotm \cite{Peri+:OSTM:Netys:2018}, \mvotm \cite{Juyal+:MVOSTM:SSS:2018}, \bto \cite [Chap. 4]{WeiVoss:TIS:2002:Morg} and \mvto \cite{Kumar+:MVTO:ICDCN:2014}) uses the concept of timestamp which helps to identify the conflicts and build the BG. For the multi-version algorithms (\mvotm and \mvto), we did not limit the number of versions because the number of \sctrn{s} in a block is finite.

We have implemented two approaches for concurrent validators,\todo{Can we remove fork-join and explain only about proposed SCV here?} First, \emph{Decentralized Validator} (Dece.) \cite{Anjana:OptSC:PDP:2019} and second \emph{Fork-join Validator} \cite{Dickerson+:ACSC:PODC:2017} as explained in \secref{intro}. Concurrent execution of SCTs by validator does not use any STM protocol; however it uses the BG given by the concurrent miner (to avoid the FBR error), which uses STMs protocols. We also proposed Smart Concurrent Validator (SCV) to detect malicious miners and prevent any malicious block from being added to the blockchain. %to execute the SCTs concurrently, correctly, and deterministically. The concurrent miner uses the STMs protocol. 
In this section, we will present the proposed SCV results. We proposed \svotm SCV, \mvotm SCV, \bto SCV, \mvto SCV, Speculative Bin SCV, and Static Bin SCV. Similarly, we called the state-of-the-art validators \cite{Anjana:OptSC:PDP:2019} as \bto Decentralized, \bto Fork-join, \mvto Decentralized, \mvto Fork-join, and Serial Validators. The results show \svotm and \mvotm validators outperform \bto, \mvto, Speculative, and Serial Validators in both the approaches. \mvotm validator executes more SCTs concurrently because the BG developed using \mvotm has fewer edges as compared to other validators.

We tested our approach with Ethereum smart contracts. Since Ethereum contracts are written in Solidity \cite{Solidity} language and are executed on the Ethereum Virtual Machine (EVM) and EVM does not support multi-threading \cite{ethereum:url,Dickerson+:ACSC:PODC:2017}. Therefore, we converted the smart contracts of Ethereum as described in Solidity documentation \cite{Solidity} into C++ multi-threaded contracts similar to the approach used by Anjana et al. \cite{Anjana:OptSC:PDP:2019}. Then we integrated them into object-based STM framework (\svotm and \mvotm) for concurrent execution of SCTs by the miners. 


\noindent
\textbf{Experimental Setup:} The experimental system consists of two sockets, each comprised of 14 cores 2.60 GHz Intel (R) Xeon (R) CPU E5-2690, and each core supports 2 hardware threads. Thus the system supports a total of 56 hardware threads. The machine runs Ubuntu 16.04.2 LTS operating system and has 32GB RAM. 


%\vspace{1mm}
\noindent
\textbf{Smart Contract Benchmarks:} We chose a diverse set of smart contracts described in Solidity documentation \cite{Solidity} as benchmarks to analyze the performance of our proposed approach. The selected benchmark contracts are (1) \emph{Coin}: a financial contract, (2) \emph{Ballot}: an electronic voting contract, (3) \emph{Simple Auction}: an auction contract, and (4) finally, a \emph{Mixed} contract: the combination of the three contracts mentioned above in equal proportion in which block consists of multiple SCTs belonging to different smart contracts. Please refer \apnref{ap-rresult} for the detailed description of benchmarks.






\noindent
\textbf{Performance Analysis:} To analyze the performance, we tested each contract under two workloads W1 and W2. (W1) The number of \sctrn{s} varies from 50 to 300 while the number of threads fixed to 50. The maximum number of SCTs in a block of Ethereum is approximately 200 \cite{Dickerson+:ACSC:PODC:2017}, but it is growing over time. (W2) The number of threads varies from 10 to 60, while the \sctrn{s} fixed at 100. The average \sctrn{s} in a block of Ethereum are around 100 \cite{EthereumAvgBlockSize}. The hash table size and shared data-items are fixed to 30 and 500 respectively for both the workloads. For accuracy, results are averaged over 26 runs in which the first run is discarded and considered as a warm-up run. Due to space constraints, here we present only Mix Contract results. The detailed analysis is given in \apnref{ap-rresult}.

\begin{wrapfigure}{!htb}{0.75\textwidth}
%\begin{figure*}%{!htb}%{0.72\textwidth}
    \centering
	\fbox
	{\includegraphics[width=.72\textwidth]{figs/w1-w2-Speedup-mix-2-2.eps}}\vspace{-.35cm}
	 \caption{Speedup of Concurrent Miners and SMVs for Mix Contract over Serial Miner and Validator on W1 and W2}
	\label{fig:w12-mix}
%\end{figure*}
\end{wrapfigure}
%\include{mixResults}


\figref{w12-mix}.(a) and \figref{w12-mix}.(b) shows the \svotm, \mvotm, \bto, \mvto, Speculative Bin, and Static Bin miners speedup over serial miner for mix contracts on workload W1 and W2 respectively. The average speedup achieved by \mvotm, \svotm, \mvto, \bto, Speculative Bin, and Static Bin miners over serial miner is 5.03$\times$, 4.47$\times$, 3.01$\times$, 2.89$\times$, 2.38$\times$, and 0.86$\times$ respectively.



As shown in \figref{w12-mix}.(a) with an increase in \sctrn{s}, the STM miners (\svotm, \mvotm, \mvto, and \bto miner) outperform Speculative Bin miner. Because the number of \sctrn{s} in the sequential bin for the Speculative Bin technique increases with an increase in \sctrn{s}. However, for lookup intensive workload and the smaller numbers of \sctrn{s} in a block, the Speculative Bin may outperform STM miners (\bto and \mvto), which can be observed in the \figref{w12-mix}.(a) at 50 \sctrn{s}.
We observed that for update intensive workload \mvotm and \svotm outperforming Speculative Bin approach. We also observed that \bto and \svotm start outperforming multi-version due to an increase in versions for update intensive workloads (for ballot contract) while increasing the number of \sctrn{s}, which in turn increases the search time to identify the correct version in \mvotm and \mvto miner. %The same reason can be applied to \mvto performance degradation over \bto.
Another observation is that the concurrent miner performances degrade for update intensive workloads with the increase in the number of \sctrn{s}.


As shown in \figref{w12-mix}.(b) for workload W2, \mvotm miner outperforms all other miners since for 100 SCTs with 500 shared data-items, the number of edges in the BG is least for \mvotm as compared to other STM miners. Another observation is that when the number of threads is less, the serial miner dominates concurrent miners. % if the workload is an update intensive.
We also calculated number of dependencies in BG by all the STM miners (shown in \figref{w1-BG} and \figref{w2depen} of \apnref{ap-rresult}). It shows that BG constructed by the \mvotm has the least number of edges for all the contracts on both the workloads. However, there is no BG for Bin based approach, so from the Block Size concern, Bin based approach is efficient, but the validator speedup is comparatively lesser then STM validators. \figref{w12-mix}.(b) and \figref{w12-mix}.(d) demonstrates that increasing the number of threads enhances the speedup till 50 threads while it decreases for 60 because our system has 56 logical threads. 

\figref{w12-mix}.(c) and \figref{w12-mix}.(d) show the speedup achieved by Smart Concurrent Validators (SCVs) over serial validator on the workloads W1 and W2, respectively. The average speedup achieved by decentralized \mvotm, \svotm, \mvto, \bto, Speculative Bin, and Static Bin decentralized SCVs are 9.87$\times$, 9.28$\times$, 8.73$\times$, 8.3$\times$, 4.14$\times$, and 3.73$\times$ over serial validator respectively.% It can be observed that the speedup achieved by Bin based SCVs is smaller compared to STM SCVs. %Therefore, for better visualisation, Y1 axis shows the speedup achieved by STM SCVs while the Y2 axis demonstrates the speedup achieved by Bin SCVs in \figref{w12-mix}.(c) and \figref{w12-mix}.(d).

It can be observed that decentralized \mvotm SCV dominates over all the other validators due to less number of edges in the BG as shown in \figref{w1-BG} of \apnref{ap-rresult}. Also, an important observation is that Bin based validators speedup is lesser than STM validators; this is because the STM validator precisely determines the concurrent STCs. For example, let a transaction $T_i$ updated a shared data-item $x$, then all other transactions that update/read/write $x$ will be kept into the Sequential Bin at miner side and, therefore, less concurrent STCs for validators. Also, the speedup achieved by a decentralized SCV is higher than the concurrent miner as the miner has to execute the \sctrn{s} concurrently using STMs (including the retries of aborted transactions) and constructs the BG. On the other hand, the validator executes the SCTs concurrently and deterministically with the help of BG (without any retries) and from the Concurrent bin for Bin based approach, respectively.



\begin{wrapfigure}{r}{0.7\textwidth}
%\begin{figure*}%{r}{0.73\textwidth}
    \centering
	\fbox{\includegraphics[width=.67\textwidth]{figs/w1-w2-mminer-mix.eps}}\vspace{-.35cm}
	\caption{{\% of average concurrent validator (Non SMV) accepted a malicious block for Mix Contract on W1 and W2}}
	%\caption{\centering Speedup of Concurrent vs Serial Miner for W1}
	\label{fig:w1w2mixmminer}
%\end{figure*}
\end{wrapfigure}


\figref{w1w2mixmminer} shows the experiments performed for the malicious miner ($mm$). A malicious miner may add an incorrect BG (i.e., EMB) in the proposed block. To solve this problem, we implemented a \emph{Smart Concurrent Validator (SCV)} to identify the $mm$ (describe in \apnref{ap-mm}). The \emph{SCV} always detects the malicious block with the help of $counter$ and straightforward reject it. \figref{w1w2mixmminer} demonstrates the percentage of validators (non-SCVs) accepting a malicious block for workload W1 and W2, respectively. Here, we consider 50 validators and run the experiments for the Mix contract. \figref{w1w2mixmminer} and represents that less than $50$\% validators are accepting a malicious block; however, during our analysis, we observed for some workload more than $50$\% validators (non-SCVs) accepted a malicious block. % However, the percentage of average STM validators accepting a malicious block is smaller compared to Bin based Validators.
Though it is a random process, even a single malicious block acceptance may create vital damage to the blockchain. So, if a malicious concurrent miner is present in the network, some validators may agree on the malicious block. The proposed \emph{SCVs} shows 100\% malicious block rejection, which serves our purpose to identify the malicious concurrent miner in the network. Another advantage of \emph{SCV} is that the validator may detect the malicious miner during the concurrent execution of malicious SCTs and need not to execute the remaining SCTs of the block, which saves the validator time.



Due to lack of space, we have shown the performance of non-SCV validators (on W1, W2) and several other experiments on W3 in \apnref{ap-rresult}. In W3, the number of shared data-items varies from 100 to 600 while the number of threads, SCTs, and hash table size are fixed to 50, 100, and 30, respectively, for all four smart contract benchmarks. The actual time (milliseconds) taken by all the miners and validators on W1 for aforementioned four smart contract benchmarks are shown from Table \ref{tab:w1-coin-miner} to Table \ref{tab:w1-mix-val} in \apnref{ap-rresult}. Along with this, we have shown the average number of dependencies in the BG and additional space required to append the BG into the block (for W1, W2, and W3) in \apnref{ap-rresult}. More details about how malicious miner propose a malicious block is presented in \apnref{ap-rresult}.






%As shown in \figref{w12-mix}.(a) after 200 \sctrn{s}, \svotm and \mvotm miner outperform then Speculative Bin miner. Because \sctrn{s} in the sequential bin for the Speculative Bin technique increases with increasing the number of \sctrn{s}. However, for lookup intensive workload, the Speculative Bin may outperform all other miners. We observed that for update intensive workload (for ballot contract), \mvotm and \svotm started outperforming Speculative Bin approach for W1. We also observed that \bto and \svotm start outperforming multi-version due to an increase in versions for update intensive workloads (for ballot contract) while increasing the number of \sctrn{s}, which in turn increases the search time to identify the correct version in \mvotm and \mvto miner. %The same reason can be applied to \mvto performance degradation over \bto.
%Another observation is that when the number of \sctrn{s} increases \bto, \mvto, and Static Bin miner performances degrade and stated doing worse than serial.

%\begin{wrapfigure}{r}{0.73\textwidth}
%\begin{figure*}%{r}{0.73\textwidth}
%    \centering
%	\fbox{\includegraphics[width=.7\textwidth]{figs/w1-w2-Speedup-mix-2-2.eps}}\vspace{-.35cm}
%   \caption{Speedup of Concurrent Miners and SMVs for Mix Contract over Serial Miner and Validator on W1 and W2}
%	\label{fig:w12-mix}
%\end{figure*}
%\end{wrapfigure}


%\figref{w12-mix}.(b) and \figref{w12-mix}.(d) demonstrates that increasing the number of threads enhances the speedup till 50 threads while it decreases for 60 because our system has 56 logical threads. As shown in \figref{w12-mix}.(b) for workload W2, Speculative Bin miner outperforms all other miners. However, \mvotm miner outperforms other STM and Static Bin miners since for 100 SCTs with 500 shared data-items, the number of edges in the BG is least for \mvotm as compared to other STM miners. Another observation is that when the number of threads is 10, serial miner dominates \bto, \mvto, and Static Bin miner. We also calculated number of dependencies in BG by all the STM miners (shown in \figref{w1-BG} and \figref{w2depen} of \apnref{ap-rresult}). It shows that BG constructed by the \mvotm has the least number of edges for all the contracts on both the workloads. However, there is no BG for Bin based approach, so from the Block Size point of view, Bin based approach will be efficient, but the validator speedup is comparatively lesser then STM validators. Further, for update intensive workloads with a fixed number of SCTs STM approach may be better than a bin based Speculative approach.



%\figref{w12-mix}.(c) and \figref{w12-mix}.(d) show the speedup achieved by Smart Concurrent Validators (SCVs) over serial validator on the workloads W1 and W2, respectively. The average speedup achieved by \emph{decentralized \mvotm, \svotm, \mvto, \bto, Speculative Bin,} and \emph{Static Bin decentralized SCVs} are {\color{blue}XXX$\times$, YYY$\times$, ZZZ$\times$, AAA$\times$, BBB$\times$, and CCC$\times$} over \emph{serial validator} respectively. The speedup achived by Bin based SCVs is smaller compared to STM SCVs. Therefore, for better visualisation, Y1 axis shows the speedup achieved by STM SCVs while the Y2 axis demonstrates the speedup achieved by Bin SCVs in \figref{w12-mix}.(c) and \figref{w12-mix}.(d).


%Decentralized \mvotm SCV dominates over all the other validators due to less number of edges in the BG as shown in \figref{w1-BG} of \apnref{ap-rresult}. Also, an important observation is that bin based validators speedup is lesser than STM validators; this is because STM validator precisely determines the concurrent STCs. For example, let a transaction $T_i$ updated a shared data-item $x$, then all other transactions that update/read/write $x$ will be kept into the Sequential bin at miner side and, therefore, less concurrent STCs for validators. The speedup achieved by a decentralized SCV is higher than the concurrent miner as the miner has to execute the \sctrn{s} concurrently using STMs (including the retries of aborted transactions) and constructs the BG. On the other hand, the validator executes the SCTs concurrently and deterministically with the help of BG (without any retries) and from the Concurrent bin for bin based approach, respectively.


%\begin{wrapfigure*}{r}{0.73\textwidth}
%\begin{figure*}%{r}{0.73\textwidth}
 %   \centering
%	\fbox{\includegraphics[width=.7\textwidth]{figs/w1-w2-mminer-mix-s.eps}}\vspace{-.35cm}
%	\caption{{\% of average concurrent validator (non SCV) accepted a malicious block for Mix Contract on W1 and W2}}
	%\caption{\centering Speedup of Concurrent vs Serial Miner for W1}
%	\label{fig:w1w2mixmminer}
%\end{figure*}
%\end{wrapfigure*}
%\figref{w1w2mixmminer} shows the experiments performed for the malicious miner ($mm$). A malicious miner may add an incorrect BG (i.e., EMB) in the proposed block. To solve this problem, we implemented a \emph{Smart Concurrent Validator (SCV)} to identify the $mm$ (describe in \apnref{ap-mm}). The \emph{SCV} always detects the malicious block with the help of $counter$ and straightforward reject it. 

%\figref{w1w2mixmminer} demonstrates the percentage of validators (non-SCVs) accepting a malicious block for workload W1 and W2, respectively. Here, we consider 50 validators and run the experiments for the Mix contract. \figref{w1w2mixmminer} and represents that more than $50$\% validators are accepting a malicious block in Bin based approach. However, the percentage of average STM validators accepting a malicious block is smaller compared to Bin based Validators. Though it is a random process, even a single malicious block acceptance may create vital damage to the blockchain. So, if a malicious concurrent miner is present in the network, some validators may agree on the malicious block. The proposed \emph{SCVs} shows 100\% malicious block rejection, which serves our purpose to identify the malicious concurrent miner in the network. Another advantage of \emph{SCV} is that the validator may detect the malicious miner during the concurrent execution of malicious SCTs and need not to execute the remaining SCTs of the block, which saves the validator time.



%Due to lack of space, we have shown the performance of non-SCV validators (on W1, W2) and several other experiments on W3 in \apnref{ap-rresult}. In W3, the number of shared data-items varies from 100 to 600 while the number of threads, SCTs, and hash table size are fixed to 50, 100, and 30, respectively, for all four smart contract benchmarks. The actual time (milliseconds) taken by all the miners and validators on W1 for aforementioned four smart contract benchmarks are shown from Table \ref{tab:w1-coin-miner} to Table \ref{tab:w1-mix-val} in \apnref{ap-rresult}. Along with this, we have shown the average number of dependencies in the BG and additional space required to append the BG into the block (for W1, W2, and W3) in \apnref{ap-rresult}. More details about how malicious miner propose a malicious block is presented in \apnref{ap-rresult}.




